Bert: Scalable Source Routed Multicast for Cloud Data Centers

Traditional IP multicast routing is not suitable for cloud data center (DC) networks due to the need for supporting large numbers of groups with large group sizes. State-of-the-art DC multicast routing approaches aim to overcome the scalability issues by, for instance, taking advantage of the symmetry of DC topologies and the programmability of DC switches to compactly encode multicast group information inside packets, thereby reducing the overhead resulting from the need to store the states of flows at the network switches. However, although these scale well with the number of multicast groups, they do not do so with group sizes, and as a result, they yield substantial traffic control overhead and network congestion. In this paper, we present Bert, a scalable, source-initiated DC multicast routing approach that scales well with both the number and the size of multicast groups, and does so through clustering, by dividing the members of the multicast group into a set of clusters with each cluster employing its own forwarding rules. Compared to the state-of-the-art approach, Bert yields much lesser traffic control overhead by significantly reducing the packet header sizes and the number of extra packet transmissions, resulting from the need for compacting forwarding rules across the switches.

==> Background.tex <==
Large-scale DCs typically are multi-rooted tree-based topologies (e.g., fat-tree~\cite{fat-tree} and its variants~\cite{vl2,f10,cft}). These types of topologies provide large numbers of parallel paths to support high bandwidth, low latency, and non-blocking connectivity among servers. 
%
The servers are tree leaves, which are connected to top-of-rack (ToR) (edge/leaf) switches. 
%
In general, DCs contain three types of switches, leaf, spine, and core, with each type residing in one layer, as shown in Fig.~\ref{fig:fig1}. At the lowest layer, leaf (aka edge) switches are interconnected through spine (aka aggregation) switches, which constitute the second layer of switches. The core switches, constituting the top/root layer, serve as connections among the spine switches. With such a DC topology, every server can communicate with any other server using the same number of hops.

%In multicast technology, rather than send multiple copies of the same data from a sender to multiple receivers, just send one copy and duplicate where paths diverge. This technology greatly reduces bandwidth consumption and transmission delay, and significantly improves application throughput. As a result, much work has gone to improve the widely used IP Multicast Routing Protocols~\cite{IPM} including IGMP~\cite{IGMP} and PIM~\cite{PIM} in the context of wide-area networks. However, in DCs, which differ in significant ways from the wide-area context, many limitations arise because when these protocols are deployed.

















